Immersive and Interactive Visualization of 3D Spatio-Temporal Data using a Space Time Hypercube

We propose an extension of the well-known Space-Time Cube (STC) visualization technique in order to visualize time-varying 3D spatial data, taking advantage of the interaction capabilities of Virtual Reality (VR). The analysis of multidimensional time-varying datasets, which size grows as recording and simulating techniques advance, faces challenges on the representation and visualization of dense data, as well as on the study of temporal variations. First, we propose the Space-Time Hypercube (STH) as an abstraction for 3D temporal data, extended from the STC concept. Second, through the example of embryo development imaging dataset, we detail the construction and visualization of a STC based on a user-driven projection of the spatial and temporal information. This projection yields a 3D STC visualization, which can also encode additional numerical and categorical data. Additionally, we propose a set of tools allowing the user to filter and manipulate the 3D STC which benefits from the visualization, exploration and interaction possibilities offered by VR. Finally, we evaluated the proposed visualization method in the context of the visualization of spatio-temporal biological data. Several biology experts accompanied the application design to provide insight on how the STC visualization could be used to explore such data. We report a user study (n=12) using non-expert users performing a set of exploration and query tasks to evaluate the system.

==> chapters/5.1.additional.examples.tex <==
%%commented on the main tex file





\section{Additional examples}\label{examples}

In this section, we present two additional examples of datasets\footnote{Details on the datasets can be found at https://morphonet.org/dataset under the names of ``Shoot-apical meristem'' and ``Sample 04''.}, also taken from the MorphoNet database, for which we generated STCs with the method previously described. 
%
The cutting plane capture resolution on these examples is 512x512. 
%
For each of the two datasets, we generated STCs based on three orthogonal cutting planes.

The first dataset shown in Figure~\ref{fig:examples}, left side, is a simulation in 42 time points of an abstract oryzalin-treated organ. The appearing outgrowth is obtained by locally softening the membrane of a shoot-apical meristem filled with uniform and steady turgor pressure. The stress magnitude on each cell, notably implied by this outgrowth, is colormapped on the STCs.
%
The second dataset, shown in Figure~\ref{fig:examples}, right side, is part of a 3D temporal imaging atlas of cell morphology for the C. elegans embryo. The recording includes 150 time points, from the 4 to 350 cells stages. The STCs displayed show the remaining lifespan of each cell as a colormap.





%\begin{figure}[t!]
%\centering
%\includegraphics[width=0.477\textwidth]{figures/elegans.pdf}
%\caption{Examples of STCs with 3 different base planes for the capture, shown on the left pictures. The original dataset, from which 3 time points are displayed on the left pictures, is part of a 3D temporal atlas of the C. elegans embryo.}\label{fig:elegans}
%\end{figure} 

